End-to-End Neuro-Symbolic Architecture for Image-to-Image Reasoning Tasks

Neural models and symbolic algorithms have recently been combined for tasks requiring both perception and reasoning. Neural models ground perceptual input into a conceptual vocabulary, on which a classical reasoning algorithm is applied to generate output. A key limitation is that such neural-to-symbolic models can only be trained end-to-end for tasks where the output space is symbolic. In this paper, we study neural-symbolic-neural models for reasoning tasks that require a conversion from an image input (e.g., a partially filled sudoku) to an image output (e.g., the image of the completed sudoku). While designing such a three-step hybrid architecture may be straightforward, the key technical challenge is end-to-end training -- how to backpropagate without intermediate supervision through the symbolic component. We propose NSNnet, an architecture that combines an image reconstruction loss with a novel output encoder to generate a supervisory signal, develops update algorithms that leverage policy gradient methods for supervision, and optimizes loss using a novel subsampling heuristic. We experiment on problem settings where symbolic algorithms are easily specified: a visual maze solving task and a visual Sudoku solver where the supervision is in image form. Experiments show high accuracy with significantly less data compared to purely neural approaches.

==> Tables/maze_results.tex <==
\begin{table}[h!]
    % \centering
    \begin{minipage}[t]{0.69\textwidth}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccc}
    \toprule 
         \multirow{2}*{\textbf{Maze dim.}} & \multicolumn{2}{c}{\textbf{Our Approach}} & \multicolumn{1}{c}{\textbf{VIN}} & 
         \multicolumn{2}{c}{\textbf{Pretrained $\mathcal{M}_e$}} \\
         \cmidrule(lr){2-3} 
         \cmidrule(lr){4-4}
         \cmidrule(lr){5-6}
         & D.A.(\%) & P.A.(\%) & P.A.(\%) & D.A.(\%) & P.A.(\%) \\ 
         \midrule
         $7\times 7$ & 99.95 & 99.4 & 96.9 & - & - \\
         $13\times 13$ & 99.91 & 99.1 & 29.2 & - & - \\ 
         $19\times 19$ & 99.96 & 97.7 & 4.4 & - & - \\ 
         $28\times 28$ & 99.81 & 95.5 & - & - & - \\ 
         $43\times 43$ & 99.89 & 93.9 & - & - & - \\
        \bottomrule
    \end{tabular}%
    }
    \label{tab:my_label}
    \end{minipage}\hspace{0.01\textwidth}
    \begin{minipage}[t]{0.29\textwidth}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccc}
    \toprule 
         $\eta$ & D.A.(\%) & P.A.(\%) \\
        \midrule
        1 & 56.80 & 0.0 \\
        1/2 & 99.94 & 98.2 \\  
        1/16 & 99.95 & 99.2 \\
        1/32 & 99.81 & 98.0 \\ 
        1/128 & 99.91 & 99.1 \\
        \bottomrule
    \end{tabular}%
    }
    \label{tab:my_label}
    \end{minipage}
    \hspace{0.5em}
    % \begin{minipage}[t]{0.25\textwidth}
    % \resizebox{\textwidth}{!}{%
    % \begin{tabular}{cccc}
    % \toprule 
    %      \multicolumn{3}{c}{\textbf{Sudoku}} \\ 
          
    %      $\eta$ & D.A.(\%) & S.A.(\%) \\
    %     \midrule
    %     1 & 11.77 & 0.0 \\
    %     1/2 & 20.92 & 0.0 \\  
    %     1/16 & 38.65 & 0.0 \\
    %     1/32 & 98.35 & 60.9 \\ 
    %     1/128 & 98.56 & 65.4 \\
    %     \bottomrule
    % \end{tabular}%
    % }
    % \label{tab:my_label}
    % \end{minipage}
     \caption{Results on \vmaze\ and \vsud\ tasks. (a) Our approach shows high input symbol classification accuracy (digit acc) and path finding accuracy, even as maze sizes increase; \VIN\ scales poorly in contrast. (b,c) Our models show significantly increased accuracy in symbol identification and task completion as subsampling proportion for policy gradient is reduced (see text for details).}
\end{table}
